Graph Convolutional Policy Network for Goal-Directed Molecular Graph Generation

Generating novel graph structures that optimize given objectives while obeying some given underlying rules is fundamental for chemistry, biology and social science research. This is especially important in the task of molecular graph generation, whose goal is to discover novel molecules with desired properties such as drug-likeness and synthetic accessibility, while obeying physical laws such as chemical valency. However, designing models to find molecules that optimize desired properties while incorporating highly complex and non-differentiable rules remains to be a challenging task. Here we propose Graph Convolutional Policy Network (GCPN), a general graph convolutional network based model for goal-directed graph generation through reinforcement learning. The model is trained to optimize domain-specific rewards and adversarial loss through policy gradient, and acts in an environment that incorporates domain-specific rules. Experimental results show that GCPN can achieve 61% improvement on chemical property optimization over state-of-the-art baselines while resembling known molecules, and achieve 184% improvement on the constrained property optimization task.

==> Graph generation with reinforcement learning/000abstract.tex <==
\begin{abstract}
Generating novel graph structures that optimize given objectives while obeying some given underlying rules is fundamental for chemistry, biology and social science research.
This is especially important in the task of molecular graph generation, whose goal is to discover novel molecules with desired properties such as drug-likeness and synthetic accessibility, while obeying physical laws such as chemical valency.
However, designing models to find molecules that optimize desired properties while incorporating highly complex and non-differentiable rules remains to be a challenging task.
Here we propose Graph Convolutional Policy Network (\name), a general graph convolutional network based model for goal-directed graph generation through reinforcement learning. The model is trained to optimize domain-specific rewards and adversarial loss through policy gradient, and acts in an environment that incorporates domain-specific rules.
Experimental results show that
\name can achieve $61\%$ improvement on chemical property optimization over state-of-the-art baselines while resembling known molecules, and achieve $184\%$ improvement on the constrained property optimization task.
\end{abstract}

==> Graph generation with reinforcement learning/010intro.tex <==
\section{Introduction}
\label{sec:intro}
% \xhdr{Why important}

% Generative machine learning models can have wide applications, as they can automatically recover the underlying data distribution without human interference. Recently, generative models have shown remarkable performance in... (images, and other more continuous domains?) \CITE  
% There has also been growing interests in building generative models over discrete data, such as natural languages\CITE and graphs\CITE. 

% In many real world applications, it can be very useful for a generative model to have the capacity to incorporate \textbf{prior knowledge}, as well as the ability to adapt to specified \textbf{desired objectives}.

% Generative models with these characteristics would be useful in many domains in the social and natural sciences.

% A particularly interesting application is molecule generation. Many important problems in drug discovery and materials science are based on the principle of designing molecules with fine-tuned structures and properties, however this remains a challenging task due to the large size and discrete nature of chemical space. For example, while the range of drug-like molecules has been estimated to be between $10^{23}$ and $10^{60}$, only approximately $10^8$ molecules have ever been made\CITE. Generative models with the ability to adapt to desired objectives present a promising way to efficiently search chemical space for molecules with desired properties.

% (Prior approaches to molecule generation have typically treated the problem as a text generation problem, by representing molecules as SMILES (simplified molecular-input line-entry system) text strings. \CITE? However text representations of molecules are very fragile, and there is often a mismatch between the similarity in the text representation of two molecules and the similarity of the actual molecular structures.)
% (Include this part?)

% Operating directly on graphs presents...

% Graph representation...?

% \xhdr{However} 

% Note that both prior knowledge and desired properties could be highly complex and non-differentiable.
% Reinforcement Learning, especially policy gradient based methods, are typically used to bypass the problem.
% There have been successes in NLP application.



Many important problems in drug discovery and material science are based on the principle of designing molecular structures with specific desired properties. However, this remains a challenging task due to the large size of chemical space. For example, the range of drug-like molecules has been estimated to be between $10^{23}$ and $10^{60}$ \cite{Polishchuk2013}. Additionally, chemical space is discrete, and molecular properties are highly sensitive to small changes in the molecular structure \cite{Kirkpatrick2004}. An increase in the effectiveness of the design of new molecules with application-driven goals would significantly accelerate developments in novel medicines and materials.

%Inverse QSAR vs first generating virtual library then using QSAR to score. Possibly mention this?

% however section...
% a lot of recent work has been done in generative models for molecules
% 1. text based representation: typical works. Many limitations with text 
% 2. graph based representation: very recent works
% however, the direct generation of molecular graphs that optimize for various desired physical, chemical and biological objectives remains to be a challenging task. 
Recently, there has been significant advances in applying deep learning models to molecule generation \cite{2017arXiv170504612J, doi:10.1021/acscentsci.7b00512, DBLP:journals/corr/abs-1712-07449, gomez2016automatic, pmlr-v70-kusner17a, dai2018syntax, Olivecrona2017, 2017ORGAN, Sanchez-Lengeling2017, 2017arXiv171000616Y}. 
%Existing methods have typically represented molecules as text sequences, such as simplified molecular-input line-entry system (SMILES) strings, which possess many disadvantages. 
%More recently, methods that can directly generate molecular graphs have been proposed. 
However, the generation of novel and valid molecular graphs that can directly optimize various desired physical, chemical and biological property objectives remains to be a challenging task, since these property objectives are highly complex \cite{Segall2012} and non-differentiable. Furthermore, the generation model should be able to actively explore the vast chemical space, as the distribution of the molecules that possess those desired properties does not necessarily match the distribution of molecules from existing datasets.
% , requiring the model able to extrapolation. 

% Existing methods utilize either SMILES text based representations, or latent space representations of pre-defined substructures to optimize desired properties. However, due to limitations of text based representations of molecules and highly complex, non-differentiable property objectives, 

% Discuss the inverse design problem? Given a property predictor, can we find molecules that have optimized properties?

% Here explain solutions and our innovation. 
\xhdr{Present Work}
In this work, we propose Graph Convolutional Policy Network (\name), an approach to generate molecules where the generation process can be guided towards specified desired objectives, while restricting the output space based on underlying chemical rules. To address the challenge of goal-directed molecule generation, we utilize and extend three ideas, namely graph representation, reinforcement learning and adversarial training, and combine them in a single unified framework. 
Graph representation learning is used to obtain vector representations of the state of generated graphs, adversarial loss is used as reward to incorporate prior knowledge specified by a dataset of example molecules, and the entire model is trained end-to-end in the reinforcement learning framework.

\xhdr{Graph representation}
We represent molecules directly as molecular graphs, which are more robust than intermediate representations such as simplified molecular-input line-entry system (SMILES) \cite{weininger1988smiles}, a text-based representation that is widely used in previous works \cite{gomez2016automatic,pmlr-v70-kusner17a,dai2018syntax,2017arXiv170504612J,doi:10.1021/acscentsci.7b00512,2017ORGAN,Sanchez-Lengeling2017}. For example, a single character perturbation in a text-based representation of a molecule can lead to significant changes to the underlying molecular structure or even invalidate it \cite{doi:10.1021/acscentsci.7b00303}. Additionally, partially generated molecular graphs can be interpreted as substructures, whereas partially generated text representations in many cases are not meaningful. As a result, we can perform chemical checks, such as valency checks, on a partially generated molecule when it is represented as a graph, but not when it is represented as a text sequence. 
% Furthermore, molecules are naturally represented as graphs, while text representations of molecules may introduce biases. For example, two similar molecules may be encoded into significantly different text representations \cite{jin2018junction}. [maybe put back when we have space]

% \todo{INCLUDE FIGURE OF A MOLECULE, ITS GRAPH, AND ITS SMILES REPRESENTATION}

\xhdr{Reinforcement learning}
A reinforcement learning approach to goal-directed molecule generation presents several advantages compared to learning a generative model over a dataset.
% generative models based on latent space.
Firstly, desired molecular properties such as drug-likeness \cite{bickerton2012quantifying, Lipinski1997} and molecule constraints such as valency are complex and non-differentiable, thus they cannot be directly incorporated into the objective function of graph generative models.
% Optimization of these properties is thus less amenable to existing approaches based on deep generative models, as such approaches cannot directly back-propagate the gradient of properties.
In contrast, reinforcement learning is capable of directly representing hard constraints and desired properties through the design of environment dynamics and reward function.
Secondly, reinforcement learning allows active exploration of the molecule space beyond samples in a dataset.
Alternative deep generative model approaches \cite{gomez2016automatic,pmlr-v70-kusner17a,dai2018syntax,jin2018junction} show promising results on reconstructing given molecules, but their exploration ability is restricted by the training dataset.

% their generalization ability often relies on the inductive bias of deep learning models \cite{neyshabur2014search}.

% Additionally, the molecular property objectives that we want to optimize are only defined for completed molecular graphs, and are more naturally treated as a delayed reward at the end of a generation process. 
%Reinforcement learning is an effective way to use delayed reward as signal to learn the best molecule generation strategy.
%Since molecular properties are highly sensitive to small changes in the molecular structure, it is challenging to estimate how good a partially generated molecular graph is. 

% Our proposed \name uses a policy gradient algorithm \cite{DBLP:journals/corr/SchulmanWDRK17} to directly optimize the terminal molecular property objectives, while incorporating chemical constraints during the molecule generation process, such as valency rules and steric strain limits. 

%The molecule generation task is treated as a sequential decision making process. 

\xhdr{Adversarial training}
% While performing goal-directed optimization of molecules, it is also crucial to ensure that the generated molecules are easy to synthesize and realistic for applications. 
Incorporating prior knowledge specified by a dataset of example molecules is crucial for molecule generation.
For example, a drug molecule is usually relatively stable in physiological conditions, non toxic, and possesses certain physiochemical properties \cite{Lin403}. Although it is possible to hand code the rules or train a predictor for one of the properties, precisely representing the combination of these properties is extremely challenging.
% that make it likely to reach its intended biological target  
% Simply optimizing the desired molecular property objective may lead to degenerate and unrealistic molecules. 
Adversarial training addresses the challenge through a learnable discriminator adversarially trained with a generator \cite{goodfellow2014generative}. After the training converges, the discriminator implicitly incorporates the information of a given dataset and guides the training of the generator.

% In \name, we leverage the idea of adversarial training \cite{goodfellow2014generative} on a dataset of example molecules known to be feasible for the application, in order to learn these feasibility properties which constrain the goal-directed graph generation process.


% meaning of feasibility:... synthesizability, toxicity, stability... hard to manually specify   
% Use known molecules as a proxy for these application specific heuristics
% We use adversarial training to constrain the possible generated molecules to be similar to...
% This is especially important in molecule generation because not all possible molecular graphs obey the physical laws of chemistry nor have realistic structures for a particular application, such as drug discovery.


\name is designed as a reinforcement learning agent (RL agent) that operates within a chemistry-aware graph generation environment. A molecule is successively constructed by either connecting a new substructure or an atom with an existing molecular graph or adding a bond to connect existing atoms.
% adding bonds between existing atoms in the partially completed molecular graph or by adding bonds between atoms in the partially completed molecular graph and new atoms.
\name predicts the action of the bond addition, and is trained via policy gradient to optimize a reward composed of molecular property objectives and adversarial loss. The adversarial loss is provided by a graph convolutional network \cite{kipf2016semi,duvenaud2015convolutional} based discriminator trained jointly on a dataset of example molecules. Overall, this approach allows direct optimization of application-specific objectives, while ensuring that the generated molecules are realistic and satisfy chemical rules.
% satisfy validity constraints and feasibility requirements. 

We evaluate \name in three distinct molecule generation tasks that are relevant to drug discovery and materials science:
molecule property optimization, property targeting and conditional property optimization. We use the ZINC dataset \cite{irwin2012zinc} to provide \name with example molecules, and train the policy network to generate molecules with high property score, molecules with a pre-specified range of target property score, or molecules containing a specific substructure while having high property score.
In all tasks, \name achieves state-of-the-art results. \name generates molecules with property scores $61\%$ higher than the best baseline method, and outperforms the baseline models in the constrained optimization setting by $184\%$ on average. 

% [save space...]
% A key observation is that compared to state-of-the-art, deep generative model based algorithms which excel at interpolating molecules, our model is capable of goal-directed optimization, which more efficiently finds novel but realistic molecules with property scores much higher than that of molecules generated by the baselines.


==> Graph generation with reinforcement learning/020related.tex <==
\section{Related Work}
\label{sec:related}

% There has been several attempts at using reinforcement learning for molecule generation. Yang et al. \cite{2017arXiv171000616Y} combined Monte Carlo tree search with a recurrent neural network (RNN) SMILES string generator to obtain molecules with optimized molecular properties. Olivecrona et al. \cite{Olivecrona2017} proposed a RNN SMILES string generator that is trained with reinforcement learning to directly optimize molecular property objectives. 
Yang et al. \cite{2017arXiv171000616Y} and Olivecrona et al. \cite{Olivecrona2017} proposed a recurrent neural network (RNN) SMILES string generator with molecular properties as objective that is optimized using Monte Carlo tree search and policy gradient respectively.
% with a recurrent neural network (RNN) SMILES string generator to obtain molecules with optimized molecular properties.  proposed a RNN SMILES string generator that is trained with reinforcement learning to directly optimize molecular property objectives. 
% Our approach also shares similarity with the models proposed by Guimaraes et al. \cite{2017ORGAN} and Sanchez-Lengeling et al. \cite{Sanchez-Lengeling2017}, where a reinforcement learning reward is combined with an adversarial loss to train a RNN SMILES string generator that can simultaneously optimize molecular property objectives while maintaining similarity to an initial set of example molecules.
Guimaraes et al. \cite{2017ORGAN} and Sanchez-Lengeling et al. \cite{Sanchez-Lengeling2017} further included an adversarial loss to the reinforcement learning reward to enforce similarity to a given molecule dataset.
In contrast, instead of using a text-based molecular representation, our approach uses a graph-based molecular representation, which leads to many important benefits as discussed in the introduction.
Jin et al. \cite{jin2018junction} proposed to use a variational autoencoder (VAE) framework, where the molecules are represented as junction trees of small clusters of atoms. This approach can only indirectly optimize molecular properties in the learned latent embedding space before decoding to a molecule, whereas our approach can directly optimize molecular properties of the molecular graphs. You et al. \cite{you2018graphrnn} used an auto-regressive model to maximize the likelihood of the graph generation process, but it cannot be used to generate attributed graphs. Li et al. \cite{li2018learning} and Li et al. \cite{2018arXiv180107299L} described sequential graph generation models where conditioning labels can be incorporated to generate molecules whose molecular properties are close to specified target scores. However, these approaches are also unable to directly perform optimization on desired molecular properties. Overall, modeling the goal-directed graph generation task in a reinforcement learning framework is still largely unexplored.

==> Graph generation with reinforcement learning/030proposed.tex <==
\section{Proposed Method}
\label{sec:proposed}

In this section we formulate the problem of graph generation as learning an RL agent that iteratively adds substructures and edges to the molecular graph in a chemistry-aware environment.
We describe the problem definition, the environment design, and the Graph Convolutional Policy Network that predicts a distribution of actions which are used to update the graph being generated.
% , the state representation of graphs with categorical node and edge types

\subsection{Problem Definition}
%We consider the problem of generating graph with features.
We represent a graph $G$ as $(A,E,F)$, where $A\in \{0, 1\}^{n\times n}$ is the adjacency matrix, and $F \in \mathbb{R}^{n\times d}$ is the node feature matrix assuming each node has $d$ features. We define $E\in \{0,1\}^{b\times n\times n}$ to be the (discrete) edge-conditioned adjacency tensor, assuming there are $b$ possible edge types. $E_{i,j,k} = 1$ if there exists an edge of type $i$ between nodes $j$ and $k$, and $A = \sum_{i=1}^b E_i$.
Our primary objective is to generate graphs that maximize a given property function $S(G) \in \mathbb{R}$, i.e., maximize $\mathbb{E}_{G'}[S(G')]$, where $G'$ is the generated graph, and $S$ could be one or multiple domain-specific statistics of interest.

It is also of practical importance to constrain our model with two main sources of prior knowledge.
(1) Generated graphs need to satisfy a set of hard constraints. 
%, i.e., restricting $G^g \in \mathcal{G}^R$. \todo{remove or define}
(2) We provide the model with a set of example graphs $G \sim p_{\mathrm{data}}(G)$, and would like to incorporate such prior knowledge by regularizing the property optimization objective with $\mathbb{E}_{G,G'}[J(G,G')]$ under distance metric $J(\cdot,\cdot)$.
In the case of molecule generation, the set of hard constraints is described by chemical valency while the distance metric is an adversarially trained discriminator.
% includes valency and steric strain limits.
% The distance metric is the distance between the chemical property distributions of the example and generated molecules.


\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{fig/GCPN.png} 
\caption{An overview of the proposed iterative graph generation method. Each row corresponds to one step in the generation process. \textbf{(a)} The state is defined as the intermediate graph $G_t$, and the set of scaffold subgraphs defined as $C$ is appended for GCPN calculation. \textbf{(b)} GCPN conducts message passing to encode the state as node embeddings then produce a policy $\pi_\theta$. \textbf{(c)} An action $a_t$ with 4 components is sampled from the policy. \textbf{(d)} The environment performs a chemical valency check on the intermediate state, and then returns \textbf{(e)} the next state $G_{t+1}$ and \textbf{(f)} the associated reward $r_t$.}
\label{fig:arch}
\end{figure}




\subsection{Graph Generation as Markov Decision Process}
% motivate why we use RL
% motivate the importance of policy network, and discuss the benefinite of our GCPN


%We adopt the approach of iterative graph generation by adding nodes and edges one at a time, without supplying the algorithm with pre-defined substructures, allowing the algorithm to fully explore the space of possible graphs. 

% describe the DP setting
A key task for building our model is to specify a generation procedure.
We designed an iterative graph generation process and formulated it as a general decision process $M=(\mathcal{S},\mathcal{A},P,R,\gamma)$, where $\mathcal{S}=\{s_i\}$ is the set of states that consists of all possible intermediate and final graphs, $\mathcal{A}=\{a_i\}$ is the set of actions that describe the modification made to current graph at each time step, $P$ is the transition dynamics that specifies the possible outcomes of carrying out an action, $p(s_{t+1}|s_t,...s_0,a_t)$. $R(s_t)$ is a reward function that specifies the reward after reaching state $s_t$, and $\gamma$ is the discount factor.
The procedure to generate a graph can then be described by a trajectory $(s_0,a_0,r_0,...,s_n,a_n,r_n)$, where $s_n$ is the final generated graph.
The modification of a graph at each time step can be viewed as a state transition distribution: $p(s_{t+1}|s_t,...,s_0) = \sum_{a_t}{p(a_t|s_t,...s_0)p(s_{t+1}|s_t,...s_0,a_t)}$, where $p(a_t|s_t,...s_0)$ is usually represented as a policy network $\pi_\theta$.

Recent graph generation models add nodes and edges based on the full trajectory $(s_t,...,s_0)$ of the graph generation procedure \cite{you2018graphrnn,li2018learning} using recurrent units, which tends to ``forget'' initial steps of generation quickly. 
% Next node and edge prediction is based on the full generation trajectory, and is often carried out with recurrent units, which tends to ``forget'' initial steps of generation quickly. 
% \bowen{check the li paper. They also propose an iterative method that does not remember the full trajectory. But they don't use RL...}
In contrast, we design a graph generation procedure that can be formulated as a Markov Decision Process (MDP), which requires the state transition dynamics to satisfy the Markov property: $p(s_{t+1}|s_t,...s_0)=p(s_{t+1}|s_t)$.
Under this property, the policy network only needs the intermediate graph state $s_t$ to derive an action (see Section \ref{sec:policy}). The action is used by the environment to update the intermediate graph being generated (see Section \ref{sec:env}).



\subsection{Molecule Generation Environment}
\label{sec:env}
% implemented using rdkit
% bond addition and atom addition
% only valid actions that do not exceed valency limits are allowed
% 
% \todo{A figure on generation procedure}
In this section we discuss the setup of molecule generation environment.
On a high level, the environment builds up a molecular graph step by step through a sequence of bond or substructure addition actions given by \name.
Figure \ref{fig:arch} illustrates the 5 main components that come into play in each step, namely state representation, policy network, action, state transition dynamics and reward.
Note that this environment can be easily extended to graph generation tasks in other settings.

\xhdr{State Space}
We define the state of the environment $s_t$ as the intermediate generated graph $G_t$ at time step $t$, which is fully observable by the RL agent. Figure \ref{fig:arch} (a)(e) depicts the partially generated molecule state before and after an action is taken. At the start of generation, we assume $G_0$ contains a single node that represents a carbon atom.

\xhdr{Action Space}
% bond addition (atom_idx_1, atom_idx_2, bond_type)
% terminal nodes
% first action is to just sample a node
% There are many potential definitions of action space for the task of sequential graph generation.
% In \cite{you2018graphrnn}, each action is defined as the adjacency vector of a new node with existing nodes on the breath first search frontier. While in \cite{li2018learning}, actions have heterogeneous types, including binary decisions of whether to add node, whether to add edge and which node an edge will connect to. \note{a bit repetitive with last part of MDP}
In our framework, we define a distinct, fixed-dimension and homogeneous action space amenable to reinforcement learning.
We design an action analogous to link prediction, which is a well studied realm in network science.
We first define a set of scaffold subgraphs $\{C_1, \ldots, C_s\}$ to be added during graph generation and the collection is defined as $C = \bigcup_{i=1}^s C_i$. 
Given a graph $G_t$ at step $t$, we define the corresponding extended graph as $G_t \cup C$.
Under this definition, an action can either correspond to connecting a new subgraph $C_i$ to a node in $G_t$ or connecting existing nodes within graph $G_t$. Once an action is taken, the remaining disconnected scaffold subgraphs are removed.
In our implementation, we adopt the most fine-grained version where $\mathcal{C}$ consists of all $b$ different single node graphs, where $b$ denotes the number of different atom types. Note that $\mathcal{C}$ can be extended to contain molecule substructure scaffolds \cite{jin2018junction}, which allows specification of preferred substructures at the cost of model flexibility.
% , at the cost of diversity of generated molecules.
In Figure \ref{fig:arch}(b), a link is predicted between the green and yellow atoms. 
%Note that the second atom selected can be either in $C$ (as in the first row), which corresponds to adding a new atom, or $G_t$ (as in the second row), which corresponds to forming a ring.
% in this case forms a ring structure in the intermediate molecular graph.
We will discuss in detail the link prediction algorithm in Section \ref{sec:policy}.

\cut{
This link prediction based action can be expressed as a vector $a_{t+1} = \textsc{concat}(a_{\mathrm{first}},a_{\mathrm{second}},a_{\mathrm{edge}},a_{\mathrm{stop}})$, where $a_{\mathrm{first}}$, $a_{\mathrm{second}}$ are the indices of selected nodes; $a_{\mathrm{edge}}$ is the predicted edge type between these two nodes; and $a_{\mathrm{stop}}$ is a binary token that decides termination of the generation procedure. We implement all these tokens with one-hot representation. Since graphs have different sizes in intermediate states, all the actions are zero padded to a maximum dimension to allow for batch training. 
This action definition implies that the molecule generation environment is deterministic, and the only randomness of the system comes from the agent's randomized policy.
}

\xhdr{State Transition Dynamics}
% We next design the state transition dynamics where domain-specific rules are incorporated.
Domain-specific rules are incorporated in the state transition dynamics. The environment carries out actions that obey the given rules. Infeasible actions proposed by the policy network are rejected and the state remains unchanged.
% , while a negative reward is given when the policy network predicts an infeasible action.
For the task of molecule generation, the environment incorporates rules of chemistry.
In Figure \ref{fig:arch}(d), both actions pass the valency check, and the environment updates the (partial) molecule according to the actions.
Note that unlike a text-based representation, the graph-based molecular representation enables us to perform this step-wise valency check, as it can be conducted even for incomplete molecular graphs.


\xhdr{Reward design}
% intermediate rewards: valency exceeding penalties
% final rewards: chemical validity, steric strain, zinc drug likeliness filters, final objective
Both intermediate rewards and final rewards are used to guide the behaviour of the RL agent. 
We define the final rewards as a sum over domain-specific rewards and adversarial rewards.
The domain-specific rewards consist of the (combination of) final property scores, such as octanol-water partition coefficient (logP), druglikeness (QED) \cite{bickerton2012quantifying} and molecular weight (MW).
Domain-specific rewards also include penalization of unrealistic molecules according to various criteria,
such as excessive steric strain and the presence of functional groups that violate ZINC functional group filters \cite{irwin2012zinc}.
The intermediate rewards include step-wise validity rewards and adversarial rewards. A small positive reward is assigned if the action does not violate valency rules, otherwise a small negative reward is assigned.
As an example, the second row of Figure \ref{fig:arch} shows the scenario that a termination action is taken. When the environment updates according to a terminating action, both a step reward and a final reward are given, and the generation process terminates.

% To improve the natural looking of generated molecules
To ensure that the generated molecules resemble a given set of molecules, we employ the Generative Adversarial Network (GAN) framework \cite{goodfellow2014generative} to define the adversarial rewards $V(\pi_{\theta},D_{\phi})$
% Specifically, we consider the following min-max game
\begin{equation}
    \min_{\theta}\max_{\phi}V(\pi_{\theta},D_{\phi}) = 
    \mathbb{E}_{x\sim p_{data}}[\log D_{\phi}(x)]+
    \mathbb{E}_{x\sim \pi_{\theta}}[\log D_{\phi}(1-x)]
\end{equation}
where $\pi_{\theta}$ is the policy network, $D_{\phi}$ is the discriminator network, $x$ represents an input graph, $p_{data}$ is the underlying data distribution which defined either over final graphs (for final rewards) or intermediate graphs (for intermediate rewards).
However, only $D_{\phi}$ can be trained with stochastic gradient descent, as $x$ is a graph object that is non-differentiable with respect to parameters $\phi$. Instead, we use $-V(\pi_{\theta},D_{\phi})$ as an additional reward together with other rewards, and optimize the total rewards with policy gradient methods \cite{yu2017seqgan} (Section \ref{sec:ppo}).
The discriminator network employs the same structure of the policy network (Section \ref{sec:policy}) to calculate the node embeddings, which are then aggregated into a graph embedding and cast into a scalar prediction.
% We apply the adversarial rewards to both the intermediate graphs and the final graphs, and the adversarial rewards are added into the intermediate rewards and final rewards respectively.




\subsection{Graph Convolutional Policy Network}
\label{sec:policy}
Having illustrated the graph generation environment, we outline the architecture of \name, a policy network learned by the RL agent to act in the environment.
\name takes the intermediate graph $G_t$ and the collection of scaffold subgraphs $C$ as inputs, and outputs the action $a_t$, which predicts a new link to be added, as described in Section \ref{sec:env}.

\xhdr{Computing node embeddings}
In order to perform link prediction in $G_t \cup C$,
our model first computes the node embeddings of an input graph using Graph Convolutional Networks (GCN) \cite{kipf2016semi,duvenaud2015convolutional,2016JCAMD..30..595K,tensor2017,DBLP:journals/corr/GilmerSRVD17}, a well-studied technique that achieves state-of-the-art performance in representation learning for molecules.
We use the following variant that supports the incorporation of categorical edge types.
The high-level idea is to perform message passing over each edge type for a total of $L$ layers. At the $l^{\text{th}}$ layer of the GCN, we aggregate all messages from different edge types to compute the next layer node embedding $H^{(l+1)} \in \mathbb{R}^{(n+c) \times k}$, where $n$, $c$ are the sizes of $G_t$ and $C$ respectively, and $k$ is the embedding dimension.
More concretely,
\begin{equation}
    H^{(l+1)} = \textsc{agg}(\text{ReLU}(\{\tilde{D}_i^{-\frac{1}{2}}\tilde{E}_i\tilde{D}_i^{-\frac{1}{2}} H^{(l)} W_i^{(l)}\}, \forall i \in (1,...,b)))
\end{equation}
where $E_i$ is the $i^{th}$ slice of edge-conditioned adjacency tensor $E$, and
$\tilde{E}_i=E_i+I$; $\tilde{D}_{i}=\sum_k\tilde{E}_{ijk}$. $W_i^{(l)}$ is a trainable weight matrix for the $i^{\text{th}}$ edge type, and $H^{(l)}$ is the node representation learned in the $l^{\text{th}}$ layer. 
We use $\textsc{agg}(\cdot)$ to denote an aggregation function that could be one of $\{\textsc{mean}, \textsc{max}, \textsc{sum}, \textsc{concat}\}$ \cite{hamilton2017inductive}. 
This variant of the GCN layer
allows for parallel implementation while remaining expressive for aggregating information among different edge types.
We apply a $L$ layer GCN to the extended graph $G_t \cup C$ to compute the final node embedding matrix $X =H^{(L)}$.
% \footnote{Note that in our case when $C$ contains single atom graphs, their node embedding computation simplifies to an embedding lookup followed by a multi-layer perceptron.}
% In practice we use a 3-layer GCN with batch normalization after each layer.
% Additionally, we observe comparable performance among different aggregation functions and select $sum(\cdot)$ for all experiments. 

\xhdr{Action prediction}
The link prediction based action $a_t$ at time step $t$ is a concatenation of four components: selection of two nodes, prediction of edge type, and prediction of termination.
Concretely, each component is sampled according to a predicted distribution governed by Equation \ref{eq:action_sampling_all} and \ref{eq:action_sampling}.
% \begin{equation}
% \label{eq:action_sampling}
% \begin{aligned}[c]
% & a_{t+1} = \textsc{concat}(a_{\mathrm{first}},a_{\mathrm{second}},a_{\mathrm{edge}},a_{\mathrm{stop}}) \\
% & f_{\mathrm{first}}(s_t) = \textsc{softmax}(m_f(X)),  \\
% & f_{\mathrm{second}}(s_t) = \textsc{softmax}(m_s(X_{a_{\mathrm{first}}},X)),  \\
% & f_{\mathrm{edge}}(s_t) = \textsc{softmax}(m_e(X_{a_{\mathrm{first}}},X_{a_{\mathrm{second}}})),  \\
% & f_{\mathrm{stop}}(s_t) = \textsc{softmax}(m_t(\textsc{agg}(X))),
% \end{aligned}
% \qquad
% \begin{aligned}[c]
% & \\
% & a_{\mathrm{first}} \sim f_{\mathrm{first}}(s_t) \in \{0,1\}^{n} \\
% & a_{\mathrm{second}} \sim f_{\mathrm{second}}(s_t) \in \{0,1\}^{n+c} \\
% & a_{\mathrm{edge}} \sim f_{\mathrm{edge}}(s_t) \in \{0,1\}^{b} \\
% & a_{\mathrm{stop}} \sim f_{\mathrm{stop}}(s_t) \in \{0,1\} 
% \end{aligned}
% \end{equation}


\begin{equation}
\label{eq:action_sampling_all}
    a_t = \textsc{concat}(a_{\mathrm{first}},a_{\mathrm{second}},a_{\mathrm{edge}},a_{\mathrm{stop}})
\end{equation}

\begin{equation}
\label{eq:action_sampling}
\begin{aligned}[c]
& f_{\mathrm{first}}(s_t) = \textsc{softmax}(m_f(X)),  \\
& f_{\mathrm{second}}(s_t) = \textsc{softmax}(m_s(X_{a_{\mathrm{first}}},X)),  \\
& f_{\mathrm{edge}}(s_t) = \textsc{softmax}(m_e(X_{a_{\mathrm{first}}},X_{a_{\mathrm{second}}})),  \\
& f_{\mathrm{stop}}(s_t) = \textsc{softmax}(m_t(\textsc{agg}(X))),
\end{aligned}
\qquad
\begin{aligned}[c]
& a_{\mathrm{first}} \sim f_{\mathrm{first}}(s_t) \in \{0,1\}^{n} \\
& a_{\mathrm{second}} \sim f_{\mathrm{second}}(s_t) \in \{0,1\}^{n+c} \\
& a_{\mathrm{edge}} \sim f_{\mathrm{edge}}(s_t) \in \{0,1\}^{b} \\
& a_{\mathrm{stop}} \sim f_{\mathrm{stop}}(s_t) \in \{0,1\} 
\end{aligned}
\end{equation}

We use $m_f$ to denote a Multilayer Perceptron (MLP) that maps $Z_{0:n} \in \mathbb{R}^{n \times k}$ to a $\mathbb{R}^{n}$ vector, which represents the probability distribution of selecting each node.
% This ensure that no nodes in the scaffold subgraphs are selected. 
The information from the first selected node $a_{\mathrm{first}}$ is incorporated in the selection of the second node by concatenating its embedding $Z_{a_{\mathrm{first}}}$ with that of each node in $G_t \cup C$.
The second MLP $m_s$ then maps the concatenated embedding to the probability distribution of each potential node to be selected as the second node.
Note that when selecting two nodes to predict a link, the first node to select, $a_{\mathrm{first}}$, should always belong to the currently generated graph $G_t$, whereas the second node to select, $a_{\mathrm{second}}$, can be either from $G_t$ (forming a cycle), or from $C$ (adding a new substructure).
To predict a link,
$m_e$ takes $Z_{a_{\mathrm{first}}}$ and $Z_{a_{\mathrm{second}}}$ as inputs and maps to a categorical edge type using an MLP. 
% Finally, the termination probability is computed by an aggregation function $\textsc{agg}$ of node embeddings into a graph embedding and an MLP $m_t$ maps the graph embedding to a scalar.
Finally, the termination probability is computed by firstly aggregating the node embeddings into a graph embedding using an aggregation function $\textsc{agg}$, and then mapping the graph embedding to a scalar using an MLP $m_t$.


\subsection{Policy Gradient Training}
\label{sec:ppo}
% supervised components. Step by step

Policy gradient based methods are widely adopted for optimizing policy networks. Here we adopt Proximal Policy Optimization (PPO) \cite{DBLP:journals/corr/SchulmanWDRK17}, one of the state-of-the-art policy gradient methods. The objective function of PPO is defined as follows
% \begin{gather}
%     L^{CLIP}(\theta)=\mathbb{E}_t[\min(r_t(\theta)\hat{A}_t,\text{clip}(r_t(\theta),1-\epsilon,1+\epsilon)\hat{A}_t)], r_t(\theta)=\frac{\pi_\theta(a_t|s_t)}{\pi_{\theta_{old}}(a_t|s_t)}\\
%     \hat{A}_t = -V_{\omega}(s_t)+r_t+\gamma r_{t+1}+...+\gamma^{T-t+1}r_{T-1}+\gamma^{T-t}V_{\omega}(s_T)
% \end{gather}
\begin{gather}
\max L^{\textsc{CLIP}}(\theta)=\mathbb{E}_t[\min(r_t(\theta)\hat{A}_t,\text{clip}(r_t(\theta),1-\epsilon,1+\epsilon)\hat{A}_t)], r_t(\theta)=\frac{\pi_\theta(a_t|s_t)}{\pi_{\theta_{old}}(a_t|s_t)}
\end{gather}
where $r_t(\theta)$ is the probability ratio that is clipped to the range of $[1-\epsilon,1+\epsilon]$, making the $L^{\textsc{CLIP}}(\theta)$ a lower bound of the conservative policy iteration objective \cite{kakade2002approximately}, $\hat{A}_t$ is the estimated advantage function which involves a learned value function $V_{\omega}(\cdot)$ to reduce the variance of estimation. In \name, $V_{\omega}(\cdot)$ is an MLP that maps the graph embedding computed according to Section \ref{sec:policy}.

It is known that pretraining a policy network with expert policies if they are available leads to better training stability and performance \cite{levine2013guided}. In our setting, any ground truth molecule could be viewed as an expert trajectory for pretraining \name.  This expert imitation objective can be written as $\min L^{\textsc{expert}}(\theta)=-\log(\pi_\theta(a_t|s_t))$, where $(s_t,a_t)$ pairs are obtained from ground truth molecules.
Specifically, given a molecule dataset, we randomly sample a molecular graph $G$, and randomly select one connected subgraph $G'$ of $G$ as the state $s_t$.
% Let $s_t$ be the state representation of $G'$.
At state $s_t$, any action that adds an atom or bond in $G\setminus G'$ can be taken in order to generate the sampled molecule.
Hence, we randomly sample $a_t \in G\setminus G'$, and use the pair $(s_t, a_t)$ to supervise the expert imitation objective.
% We train \name to maximize the likelihood of these observed $(s_t,a_t)$ pairs.

==> Graph generation with reinforcement learning/040experiments.tex <==
\section{Experiments}
\label{sec:experiments}


% To demonstrate effectiveness of the learned policy network and the quality of generated molecules, we compare our method with state-of-the-art molecule generation algorithms in the following tasks.
% , and analyze the importance of each \name component.
To demonstrate effectiveness of goal-directed search for molecules with desired properties,
we compare our method with state-of-the-art molecule generation algorithms in the following tasks.

\xhdr{Property Optimization} The task is to generate novel molecules whose specified molecular properties are optimized. This can be useful in many applications such as drug discovery and materials science, where the goal is to identify molecules with highly optimized properties of interest.

%% delete
% For example, a suitable drug candidate should be a very potent binder of the desired biological target.

\xhdr{Property Targeting} The task is to generate novel molecules whose specified molecular properties are as close to the target scores as possible. This is crucial in generating virtual libraries of molecules with properties that are generally suitable for a desired application. For example, a virtual molecule library for drug discovery should have high drug-likeness and synthesizability. 
% molecular weight (MW), octanol-water partition coefficient (logP) and quantitative estimate of drug-likeness (QED).

% \xhdr{Property Imitation} \note{name okay?} Given an example set of molecules, the task is to generate novel molecules whose chemical properties are similar to that of the example set of molecules. This can be useful for expanding the size of an existing virtual library of molecules.

\xhdr{Constrained Property Optimization}
The task is to generate novel molecules whose specified molecular properties are optimized, while also containing a specified molecular substructure. This can be useful in lead optimization problems in drug discovery and materials science, where we want to make modifications to a promising lead molecule and improve its properties \cite{Bleicher2003}.
% In drug discovery, people usually modify a given molecule to optimize for some desired properties.
% We formulate the task as constraining the optimized molecule to contain a given molecule substructure. 
%The task is attempted in \cite{jin2018junction}, yet their approach cannot guarantee generated molecules contain a given structure. In the experiment, we select the same 800 molecules that is used in \cite{jin2018junction} as scaffolds, and optimized for the penalized logP score.


% \note {possible work on structure constrained property optimization, either start from a original molecule, or have a similarity based reward to an original molecule }


% \begin{table}[t]
% % \parbox{.45\linewidth}{
% \centering
% \begin{tabular}{c | c c c c | c c c c }
% 	\toprule
% 	Method & \multicolumn{4}{c}{Penalized logP} & \multicolumn{4}{c}{QED} \\
% 	 &1st & 2nd & 3rd & Validity &1st & 2nd & 3rd & Validity\\
% 	\midrule
% 	ZINC & $4.52$ & $4.30$ & $4.23$ & $100.0\%$ & $0.948$ & $0.948$ & $0.948$ & $100.0\%$ \\
% 	\midrule
% 	ORGAN & $3.63$ & $3.49$ & $3.44$ & $0.4\%$ & $0.896$ & $0.824$ & $0.820$ & $2.2\%$ \\
% 	JT-VAE & $5.30$ & $4.93$ & $4.49$ & $100.0\%$ & $0.925$ & $0.911$ & $0.910$ & $100.0\%$ \\
% 	\name & $\textbf{7.98}$ & $\textbf{7.85}$ & $\textbf{7.80}$ & $\textbf{100.0\%}$ & $\textbf{0.948}$ & $\textbf{0.947}$ & $\textbf{0.946}$ & $\textbf{100.0\%}$  \\
% 	GCPN\textsubscript{plain}  & $23.88^*$ & $23.88^*$ & $23.87^*$ & $100.0\%$ & $0.936$ & $0.932$ & $0.926$ & $100.0\%$ \\
% 	\bottomrule
% \end{tabular}
% \caption{Comparison of the top 3 property scores of generated molecules found by each model.
% }
% \label{tab:top3_comparison}
% \vspace{-4mm}
% \end{table}





\subsection{Experimental Setup}

We outline our experimental setup in this section. Further details are provided in the appendix\footnote{Link to code and datasets: \url{https://github.com/bowenliu16/rl_graph_generation}}.

\xhdr{Dataset}
For the molecule generation experiments, we utilize the ZINC250k molecule dataset \cite{irwin2012zinc} that contains 250,000 drug like commercially available molecules whose maximum atom number is 38. 
We use the dataset for both expert pretraining and adversarial training.

\xhdr{Molecule environment}
% Some molecule statistics are scaled with the molecule size. To make a fair comparison with existing approaches, we set the maximum number of atom for generated molecule to be 38, which equals the max molecule size in ZINC.
We set up the molecule environment as an OpenAI Gym environment \cite{DBLP:journals/corr/BrockmanCPSSTZ16} using RDKit \cite{landrum2006rdkit} and adapt it to the ZINC250k dataset. Specifically, the maximum atom number is set to be 38. There are 9 atom types and 3 edge types, as molecules are represented in kekulized form. 
% where the aromatic bonds are kekulized to double bonds. 
% We design the reward such that empirically the ratio of intermediate valency reward, intermediate adversarial reward, final adversarial reward, final chemical filter reward and final chemical property reward is roughly $1:1:1:2:4$ when those rewards reach their optimal value.
For specific reward design, we linearly scale each reward component according to its importance in molecule generation from a chemistry point of view as well as the quality of generation results. When summing up all the rewards collected from a molecule generation trajectory, the range of the reward value that the model can get is $[-4,4]$ for final chemical property reward, $[-2,2]$ for final chemical filter reward, $[-1,1]$ for final adversarial reward, $[-1,1]$ for intermediate adversarial reward and $[-1,1]$ for intermediate validity reward.

\xhdr{\name Setup}
We use a 3-layer defined \name as the policy network with $64$ dimensional node embedding in all hidden layers, and batch normalization \cite{pmlr-v37-ioffe15} is applied after each layer. Another 3-layer GCN with the same architecture is used for discriminator training. We find little improvement when further adding GCN layers.
We observe comparable performance among different aggregation functions and select $\textsc{sum}(\cdot)$ for all experiments. We found both the expert pretraining and RL objective important for generating high quality molecules, thus both of them are kept throughout training.
Specifically, we use PPO algorithm to train the RL objective with the default hyperparameters as we do not observe too much performance gain from tuning these hyperparameters, and the learning rate is set as 0.001. The expert pretraining objective is trained with a learning rate of 0.00025, and we do observe that adding this objective contributes to faster convergence and better performance.
Both objectives are trained using Adam optimizer \cite{kingma2014adam} with batch size 32.







\xhdr{Baselines}
We compare our method with the following state-of-the-art baselines.
%(Other possible baselines: charvae, grammarvae, sdvae, ChemTS, "Population based denovo molecule generation using grammatical evolution)
Junction Tree VAE (JT-VAE) \cite{jin2018junction} is a state-of-the-art algorithm that combines graph representation and a VAE framework for generating molecular graphs, 
and uses Bayesian optimization over the learned latent space to search for molecules with optimized property scores.
% It uses junction trees of clusters of atoms as intermediate representations of molecules to be encoded in the latent space. [we should have discussed this in related work]
JT-VAE has been shown to outperform previous deep generative models for molecule generation, including Character-VAE \cite{gomez2016automatic}, Grammar-VAE \cite{pmlr-v70-kusner17a}, SD-VAE \cite{dai2018syntax} and GraphVAE \cite{simonovsky2018graphvae}.
We also compare our approach with 
ORGAN \cite{2017ORGAN}, a state-of-the-art RL-based molecule generation algorithm using a text-based representation of molecules.
% , whose policy uses SMILE string representations of molecules to predict the next character to be added to the string. [we should have discussed this in related work]
% We run both baselines using their released code and tune the hyper-parameters such that all the tasks can be finished within manageable time.
To demonstrate the benefits of learning-based approaches, we further implement a simple rule based model using the stochastic hill-climbing algorithm.
% and compare it with the proposed model in an experiment to optimize QED score. 
We start with a graph containing a single atom (the same setting as GCPN), traverse all valid actions given the current state, randomly pick the next state with top 5 highest property score as long as there is improvement over the current state, and loop until reaching the maximum number of nodes.
To make fair comparison across different methods, we set up the same objective functions for all methods, and run all the experiments on the same computing facilities using 32 CPU cores. We run both deep learning baselines using their released code and allow the baselines to have wall clock running time for roughly 24 hours, while our model can get the results in roughly 8 hours.

% , and implementations details are discussed in the appendix.

% \todo{baseline configurations}

% \rex{Need experimental setup (hyper-param) for \name here }

\begin{table}[t]
\centering		
\caption{Comparison of the top 3 property scores of generated molecules found by each model.}
\label{tab:top3_comparison}
\resizebox{0.85\columnwidth}{!}{ \renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}clcccccccc@{}}\cmidrule[\heavyrulewidth]{2-10}
& \multirow{3}{*}{\vspace*{8pt}Method}&\multicolumn{4}{c}{Penalized logP} & \multicolumn{4}{c}{QED}\\ \cmidrule{3-10}
& &1st & 2nd & 3rd & Validity &1st & 2nd & 3rd & Validity
\\ \cmidrule{2-10}

	& ZINC & $4.52$ & $4.30$ & $4.23$ & $100.0\%$ & $0.948$ & $0.948$ & $0.948$ & $100.0\%$ \\
	\cmidrule{2-10}
	& Hill Climbing & $-$ & $-$ & $-$ & $-$ & $0.838$ & $0.814$ & $0.814$ & $100.0\%$ \\
	\cmidrule{2-10}
	& ORGAN & $3.63$ & $3.49$ & $3.44$ & $0.4\%$ & $0.896$ & $0.824$ & $0.820$ & $2.2\%$ \\
	& JT-VAE & $5.30$ & $4.93$ & $4.49$ & $100.0\%$ & $0.925$ & $0.911$ & $0.910$ & $100.0\%$ \\
	& \name & $\textbf{7.98}$ & $\textbf{7.85}$ & $\textbf{7.80}$ & $\textbf{100.0\%}$ & $\textbf{0.948}$ & $\textbf{0.947}$ & $\textbf{0.946}$ & $\textbf{100.0\%}$  \\
\cmidrule[\heavyrulewidth]{2-10}
\end{tabular}}
% \vspace{-4mm}
\end{table}


\subsection{Molecule Generation Results}
\xhdr{Property optimization}
In this task, we focus on generating molecules with the highest possible penalized logP \cite{pmlr-v70-kusner17a} and QED \cite{bickerton2012quantifying} scores. Penalized logP is a logP score that also accounts for ring size and synthetic accessibility \cite{ertlestimation}, while QED is an indicator of drug-likeness. 
Note that both scores are calculated from empirical prediction models whose parameters are estimated from related datasets \cite{doi:10.1021/ci990307l,bickerton2012quantifying}, and these scores are widely used in previous molecule generation papers \cite{gomez2016automatic,pmlr-v70-kusner17a,dai2018syntax,simonovsky2018graphvae,2017ORGAN}.
Penalized logP has an unbounded range, while the QED has a range of $[0,1]$ by definition, thus directly comparing the percentage improvement of QED may not be meaningful. We adopt the same evaluation method in previous approaches \cite{pmlr-v70-kusner17a,dai2018syntax,jin2018junction}, reporting the best 3 property scores found by each model and the fraction of molecules that satisfy chemical validity. 
Table \ref{tab:top3_comparison} summarizes the best property scores of molecules found by each model, and the statistics in ZINC250k is also shown for comparison. 
Our method consistently performs significantly better than previous methods when optimizing penalized logP, achieving an average improvement of $61\%$ compared to JT-VAE, and $186\%$ compared to ORGAN. Our method outperforms all the baselines in the QED optimization task as well, and significantly outperforms the stochastic hill climbing baseline.

Compared with ORGAN, our model can achieve a perfect validity ratio due to the molecular graph representation that allows for step-wise chemical valency check. Compared to JT-VAE, our model can reach a much higher score owing to the fact that RL allows for direct optimization of a given property score and is able to easily extrapolate beyond the given dataset.
Visualizations of generated molecules with optimized logP and QED scores are displayed in Figure \ref{fig:mol}(a) and (b) respectively.

Although most generated molecules are realistic, in some very rare cases, especially where we reduce the  of the adversarial reward and expert pretraining components, our method can generate undesirable molecules with astonishingly high penalized logP predicted by the empirical model, such as the one on the bottom-right of Figure \ref{fig:mol}(a) in which our method correctly identified that Iodine has the highest per atom contribution in the empirical model used to calculate logP. These undesirable molecules are likely to have inaccurate predicted properties and illustrate an issue with optimizing properties calculated by an empirical model, such as penalized logP and QED, without incorporating prior knowledge. Empirical prediction models that predict molecular properties generalize poorly for molecules that are significantly different from the set of molecules used to train the model. Without any restrictions on the generated molecules, an optimization algorithm would exploit the lack of generalizability of the empirical property prediction models in certain areas of molecule space. Our model addresses this issue by incorporating prior knowledge of known realistic molecules using adversarial training and expert pretraining, which results in more realistic molecules, but with lower property scores calculated by the empirical prediction models.
Note that the hill climbing baseline algorithm mostly generates undesirable cases where the accuracy of the empirical prediction model is questionable, thus its performance with optimizing penalized logP is not listed on Table \ref{tab:top3_comparison}.

% Unlike previous methods, \name is able to identify these exceptional cases that reveal the flaw of the unbounded penalized logP score.

% certain algorithms are good at exploiting 
% the models predict high penalized log p with a large uncertainty that is not captured by the RL.
% change degenerate. We want to avoid molecules that exploit the poor generalizability of the empirical prediction model
% undesirable vs unrealistic

% \rex{more observations depending on results}
% \jiaxuan{emphasize extrapolation ability}

% Jiaxuan merged this into introduction
% In VAE-based approaches, property optimization is indirectly achieved via Bayesian optimization on the latent space learned by the VAE. However, the approach highly relies on the quality of the learned latent space and could be biased.
% In contrast, RL-based approaches are able to directly optimize the property score through incorporating it to the reward, and optimize end-to-end without bias.

% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|cc|cc|cc|cc}
% 	\toprule
% 	Method & \multicolumn{2}{c}{$-2.5\leq\text{logP}\leq -2$} & \multicolumn{2}{c}{$5\leq\text{logP}\leq 5.5$} & \multicolumn{2}{c}{$150\leq\text{MW}\leq 200$} & \multicolumn{2}{c}{$500\leq\text{MW}\leq 550$} \\
% 	 &Success & Diversity  &Success & Diversity  &Success & Diversity &Success & Diversity \\
% 	\midrule
% 	ZINC & $0.3\%$ & $0.919$ & $1.3\%$ & $0.909$ & $1.7\%$ & $0.938$ & $0$ & $-$ \\
% 	\midrule
% 	JT-VAE & $11.3\%$ & $\textbf{0.846}$ & $7.6\%$ & $0.907$ & $0$ & $-$ & $16.0\%$ & $0.898$ \\
% 	ORGAN & $0$ & - & $0.2\%$ & $\textbf{0.909}$ & $15.1\%$ & $0.759$ & $0.1\%$ & $0.907$ \\
% 	\name & $\textbf{85.5\%}$ & $0.392$ & $\textbf{54.7\%}$ & $0.855$ & $76.1\%$ & $\textbf{0.921}$ & $\textbf{74.1}\%$ & $\textbf{0.920}$  \\
% 	\bottomrule
% \end{tabular}
% }
% \caption{Comparison of the effectiveness of property targeting task.
% }
% \label{tab:target}
% \vspace{-4mm}

% \end{table}


\begin{table}[t]
\centering		
\caption{Comparison of the effectiveness of property targeting task.}
\label{tab:target}
\resizebox{\columnwidth}{!}{ \renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}clcccccccc@{}}\cmidrule[\heavyrulewidth]{2-10}
& \multirow{3}{*}{\vspace*{8pt}Method}&\multicolumn{2}{c}{$-2.5\leq\text{logP}\leq -2$}&\multicolumn{2}{c}{$5\leq\text{logP}\leq 5.5$}&\multicolumn{2}{c}{$150\leq\text{MW}\leq 200$}&\multicolumn{2}{c}{$500\leq\text{MW}\leq 550$}\\ \cmidrule{3-10}
& & Success & Diversity  &Success & Diversity  &Success & Diversity &Success & Diversity
\\ \cmidrule{2-10}

	& ZINC & $0.3\%$ & $0.919$ & $1.3\%$ & $0.909$ & $1.7\%$ & $0.938$ & $0$ & $-$ \\
	\cmidrule{2-10}
	& JT-VAE & $11.3\%$ & $\textbf{0.846}$ & $7.6\%$ & $0.907$ & $0.7\%$ & $0.824$ & $16.0\%$ & $0.898$ \\
	& ORGAN & $0$ & $-$ & $0.2\%$ & $\textbf{0.909}$ & $15.1\%$ & $0.759$ & $0.1\%$ & $0.907$ \\
	& \name & $\textbf{85.5\%}$ & $0.392$ & $\textbf{54.7\%}$ & $0.855$ & $\textbf{76.1\%}$ & $\textbf{0.921}$ & $\textbf{74.1}\%$ & $\textbf{0.920}$  \\
\cmidrule[\heavyrulewidth]{2-10}
\end{tabular}}
% \vspace{-4mm}
\end{table}





% \begin{table}[t]
% \centering
% \begin{tabular}{c | c c c | c c c}
% 	\toprule
% 	$\delta$ & \multicolumn{3}{c}{JT-VAE} & \multicolumn{3}{c}{\name}\\
% 	 &Improvement & Similarity  & Success & Improvement & Similarity  & Success \\
% 	\midrule
% 	0.0 & $1.91\pm 2.04$ & $0.28\pm 0.15$ & $97.5\%$ & $\mathbf{4.20\pm 1.28}$ & $\mathbf{0.32\pm 0.12}$ & $\mathbf{100.0\%}$  \\
% 	0.2 & $1.68\pm 1.85$ & $0.33\pm 0.13$ & $97.1\%$ & $\mathbf{4.12\pm 1.19}$ & $\mathbf{0.34\pm 0.11}$ & $\mathbf{100.0\%}$  \\
% 	0.4 & $0.84\pm 1.45$ & $\mathbf{0.51\pm 0.10}$ & $83.6\%$ & $\mathbf{2.49\pm 1.30}$ & $0.47\pm 0.08$ & $\mathbf{100.0\%}$  \\
% 	0.6 & $0.21\pm 0.71$ & $0.69\pm 0.06$ & $46.4\%$ & $\mathbf{0.79\pm 0.63}$ & $\mathbf{0.68\pm 0.08}$ & $\mathbf{100.0\%}$  \\
% 	\bottomrule
% \end{tabular}
% \caption{Comparison of the performance in constrained optimization task.
% }
% \label{tab:conditional}
% \vspace{-4mm}
% \end{table}


\begin{table}[t]
\centering		
\caption{Comparison of the performance in the constrained optimization task.}
\label{tab:conditional}
\resizebox{0.9\columnwidth}{!}{ \renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}clcccccc@{}}\cmidrule[\heavyrulewidth]{2-8}
& \multirow{3}{*}{\vspace*{8pt}$\delta$}&\multicolumn{3}{c}{JT-VAE}&\multicolumn{3}{c}{\name}\\\cmidrule{3-8}
& & {Improvement} & {Similarity} & {Success}& {Improvement} & {Similarity} & {Success}
\\ \cmidrule{2-8}
& 0.0 & $1.91\pm 2.04$ & $0.28\pm 0.15$ & $97.5\%$ & $\mathbf{4.20\pm 1.28}$ & $\mathbf{0.32\pm 0.12}$ & $\mathbf{100.0\%}$  \\
& 0.2 & $1.68\pm 1.85$ & $0.33\pm 0.13$ & $97.1\%$ & $\mathbf{4.12\pm 1.19}$ & $\mathbf{0.34\pm 0.11}$ & $\mathbf{100.0\%}$  \\
& 0.4 & $0.84\pm 1.45$ & $\mathbf{0.51\pm 0.10}$ & $83.6\%$ & $\mathbf{2.49\pm 1.30}$ & $0.47\pm 0.08$ & $\mathbf{100.0\%}$  \\
& 0.6 & $0.21\pm 0.71$ & $0.69\pm 0.06$ & $46.4\%$ & $\mathbf{0.79\pm 0.63}$ & $\mathbf{0.68\pm 0.08}$ & $\mathbf{100.0\%}$  \\   
\cmidrule[\heavyrulewidth]{2-8}
\end{tabular}}
% \vspace{-4mm}
\end{table}




\begin{figure}[h]
% \vspace{-4mm}
\centering
\includegraphics[width=\linewidth]{fig/mol} 
\caption{Samples of generated molecules in property optimization and constrained property optimization task. In \textbf{(c)}, the two columns correspond to molecules before and after modification.}
\label{fig:mol}
% \vspace{-4mm}
\end{figure}







% \begin{figure}[h]
 
% \begin{subfigure}{0.19\textwidth}
% \includegraphics[width=\linewidth]{fig/mol_logp_normal.png} 
% \caption{\name}
% \label{fig:subim1}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
% \includegraphics[width=\linewidth]{fig/mol_logp_nogan.png}
% \caption{\name without GAN}
% \label{fig:subim2}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
% \includegraphics[width=\linewidth]{fig/mol_logp_nofilter.png} 
% \caption{\name without filter}
% \label{fig:subim1}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
% \includegraphics[width=\linewidth]{fig/mol_logp_nofilter.png} 
% \caption{constrained optimization before \jiaxuan{placeholder}}
% \label{fig:subim1}
% \end{subfigure}
% \begin{subfigure}{0.19\textwidth}
% \includegraphics[width=\linewidth]{fig/mol_logp_nofilter.png} 
% \caption{constrained optimization after \jiaxuan{placeholder}}
% \label{fig:subim1}
% \end{subfigure}
% \caption{Visualization of molecule with top scores \jiaxuan{we will show more molecules}}
% \label{fig:image2}
% \end{figure}


\xhdr{Property Targeting}
In this task, we specify a target range for molecular weight (MW) and logP, and 
report the percentage of generated molecules with property scores within the range, as well as the diversity of generated molecules.
The diversity of a set of molecules is defined as the average pairwise Tanimoto distance between the Morgan fingerprints \cite{rogers2010extended} of the molecules.
The RL reward for this task is the L1 distance between the property score of a generated molecule and the range center.
To increase the difficulty, we set the target range such that few molecules in ZINC250k dataset are within the range to test the extrapolation ability of the methods to optimize for a given target. The target ranges include $-2.5\leq\text{logP}\leq -2$, $5\leq\text{logP}\leq 5.5$, $150\leq\text{MW}\leq 200$ and $500\leq\text{MW}\leq 550$. 

As is shown in Table \ref{tab:target}, \name has a significantly higher success rate in generating molecules with properties within the target range, compared to baseline methods.
In addition, \name is able to generate molecules with high diversity, indicating that it is capable of learning a general stochastic policy to generate molecular graphs that fulfill the property requirements.


% In figure ???, we plot the distribution of three properties of generated molecules, namely molecular weight, logP and QED. \rex{write some stuff after results}

% % decide not putting this as it is not for Goal-directed molecule generation
% \xhdr{Property Imitation}
% In this task, there is no explicit predictor for the desired property. Instead, the model needs to acquire the knowledge from a training set of molecules.
% We first pre-train the policy network using the training set of molecules \rex{more details later}, and set the reward to be the adversarial loss introduced in Section \ref{sec:env}.

% To evaluate the similarity of molecules in training set and molecules generated by each model, we plot the distributions of a variety of molecule properties in the training set and generated set of molecules.
% Earth-mover distance is used to compute a distance between these distributions.


\xhdr{Constrained Property Optimization}
% To conduct constrained optimization, we can simply initialize the molecule environment with some given desirable molecules, then conduct training with desirable properties as reward.
In this experiment, we optimize the penalized logP while constraining the generated molecules to contain one of the 800 ZINC molecules with low penalized logP, following the evaluation in JT-VAE. Since JT-VAE cannot constrain the generated molecule to have certain structure, we adopt their evaluation method where the constraint is relaxed such that the molecule similarity $sim(G,G')$ between the original and modified molecules is above a threshold $\delta$. 
% We also use the Tanimoto distance to compute molecule similarity.

% We run the evaluation 800 times, initializing the molecule state to be each one of the 800 ZINC molecules, then conduct the same training procedure as property optimization task. Mean and standard deviation of property score improvement and similarity are reported in Table \ref{tab:conditional}.
We train a fixed \name in an environment whose initial state is randomly set to be one of the 800 ZINC molecules, then conduct the same training procedure as the property optimization task. Over the 800 molecules, the mean and standard deviation of the highest property score improvement and the corresponding similarity between the original and modified molecules are reported in Table \ref{tab:conditional}.
Our model significantly outperforms JT-VAE with 184\% higher penalized logP improvement on average, and consistently succeeds in discovering molecules with higher logP scores.
Also note that JT-VAE performs optimization steps for each given molecule constraint. In contrast, \name can generalize well: it learns a general policy to improve property scores, and applies the same policy to all 800 molecules.
Figure \ref{fig:mol}(c) shows that \name can modify ZINC molecules to achieve high penalized logP score while still containing the substructure of the original molecule.


% \subsection{maintaining naturalness of generated molecules}
% % \jiaxuan{let's decide later whether to have this}
% We also conduct ablation studies and consider variants of \name, by removing the adversarial loss and pre-training component respectively. 

% % \subsection{General Setting of Graph Generation}
% % \rex{let's decide later whether to have this, depending on the overall progress}
% % We show the strong performance of \name when solving the graph generation problem in the most general setting without domain-specific constraints. 
% % When specifying a target power-law degree distribution, \name generates graphs whose degree distribution matches very closely to the target degree distribution.

% % We also demonstrate that \name can generate graphs similar to those in a given training set. 




%%% If we have space...
% \subsection{Interpreting Learned Policies}



==> Graph generation with reinforcement learning/050conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We introduced \name, a graph generation policy network using graph state representation and adversarial training, and applied it to the task of goal-directed molecular graph generation. \name consistently outperforms other state-of-the-art approaches in the tasks of molecular property optimization and targeting, and at the same time, maintains $100\%$ validity and resemblance to realistic molecules. Furthermore, the application of \name can extend well beyond molecule generation. The algorithm can be applied to generate graphs in many contexts, such as electric circuits, social networks, and explore graphs that can optimize certain domain specific properties.

==> Graph generation with reinforcement learning/acknowledgements.tex <==
% \section{Conflict of Interest}



\section{Acknowledgements}
The authors thank Xiang Ren, Marinka Zitnik, Jiaming Song, Joseph Gomes, Amir Barati Farimani, Peter Eastman, Franklin Lee, Zhenqin Wu and Paul Wender for their helpful discussions. This research has been supported in part by DARPA SIMPLEX, ARO MURI, Stanford Data Science Initiative, Huawei, JD, and Chan Zuckerberg Biohub.
The Pande Group acknowledges the generous support of Dr.  Anders G. Frøseth and Mr. Christian Sundt for our work on machine learning.  The Pande Group is broadly supported by grants from the NIH (R01 GM062868 and U19 AI109662) as well as gift funds and contributions from Folding@home donors.

V.S.P. is a consultant \& SAB member of Schrodinger, LLC and Globavir, sits on the Board of Directors of Apeel Inc, Asimov Inc, BioAge Labs, Freenome Inc, Omada Health, Patient Ping, Rigetti Computing,  and  is  a  General  Partner  at  Andreessen Horowitz. 

==> Graph generation with reinforcement learning/micro.tex <==
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}
\usepackage{url}
\usepackage{verbatim} % allows multiline comments
\usepackage{graphicx}
\usepackage{caption} 
\usepackage{multirow}
%\usepackage{algorithm}
%\usepackage[noend]{algorithmic}
\usepackage[linesnumbered,ruled]{algorithm2e}
\usepackage{xspace}
\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{times}
\usepackage{xr}
\usepackage{bbm}
\usepackage{bm}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{hyperref}       % hyperlinks
\usepackage{multicol}

\usepackage{perpage} %the perpage package
\MakePerPage{footnote} %the perpage package command

\newcommand{\note}[1]{{{\textcolor{blue}{[note: #1]}}}}
\newcommand{\jure}[1]{{{\textcolor{red}{[Jure: #1]}}}}
\newcommand{\rex}[1]{{{\textcolor{magenta}{[Rex: #1]}}}}
\newcommand{\bowen}[1]{{{\textcolor{orange}{[Bowen: #1]}}}}
\newcommand{\jiaxuan}[1]{{{\textcolor{green}{[Jiaxuan: #1]}}}}

\newcommand{\xhdr}[1]{{\noindent\bfseries #1}.}
\newcommand{\todo}[1]{{\textcolor{red}{TODO: #1}}}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\CITE}{{\textcolor{red}{[CITE]}}}
\newcommand{\name}{GCPN\xspace}

\newcommand{\V}{\mathcal{V}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\G}{\mathcal{G}}


\newcommand{\nedge}{k}
\newcommand{\mb}{\mathbf}
% \newcommand{\mc}{\mathcal}
\newcommand{\cut}[1]{}
%\newcommand{\xhdr}[1]{\vspace{1.7mm}\noindent{{\bf #1}}}
\newcommand{\casc}{{\mathbf{t}}}
\newcommand{\alphs}{{\mathbf{A}}}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{observation}{\textbf{Observation}}
\newcommand{\xsketch}{\noindent {\it Proof Sketch.}}
\newcommand{\netinf}{{\textsc{Net\-Inf}}\xspace}
\newcommand{\multitree}{{\textsc{Multi\-Tree}}\xspace}
\newcommand{\netrate}{{\textsc{Net\-Rate}}\xspace}
\newcommand{\connie}{{\textsc{Co\-nNIe}}\xspace}
\newcommand{\maxinf}{{\textsc{Max\-Inf}}\xspace}
\newcommand{\expo}{{\textsc{Exp}}\xspace}
\newcommand{\pow}{{\textsc{Pow}}\xspace}
\newcommand{\ray}{{\textsc{Ray}}\xspace}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\unobs}{{\infty}}
\newcommand\T{\rule{0pt}{2.6ex}}
\newcommand\B{\rule[-1.2ex]{0pt}{0pt}}
\DeclareMathOperator*{\argmax}{argmax}

\newcommand{\ba}{Barab\'asi-Albert }
\newcommand{\er}{Erd\H{o}s-R\'enyi}
\newcommand{\angstrom}{\textup{\AA}}
\newcommand{\mmd}{\mathrm{MMD}}
\newcommand{\graphrnnmlp}{GraphRNN-S}
\newcommand{\graphrnnrnn}{GraphRNN}

